FinGPT-HPC: Efficient Pretraining and Finetuning Large Language Models for Financial Applications with High-Performance Computing

Large language models (LLMs) are computationally intensive. The computation workload and the memory footprint grow quadratically with the dimension (layer width). Most of LLMs' parameters come from the linear layers of the transformer structure and are highly redundant. These linear layers contribute more than 80% of the computation workload and 99% of the model size. To pretrain and finetune LLMs efficiently, there are three major challenges to address: 1) reducing redundancy of the linear layers; 2) reducing GPU memory footprint; 3) improving GPU utilization when using distributed training. Prior methods, such as LoRA and QLoRA, utilized low-rank matrices and quantization to reduce the number of trainable parameters and model size, respectively. However, the resulting model still consumes a large amount of GPU memory. In this paper, we present high-performance GPU-based methods that exploit low-rank structures to pretrain and finetune LLMs for financial applications. We replace one conventional linear layer of the transformer structure with two narrower linear layers, which allows us to reduce the number of parameters by several orders of magnitude. By quantizing the parameters into low precision (8-bit and 4-bit), the memory consumption of the resulting model is further reduced. Compared with existing LLMs, our methods achieve a speedup of 1.3X and a model compression ratio of 2.64X for pretaining without accuracy drop. For finetuning, our methods achieve an average accuracy increase of 6.3% and 24.0% in general tasks and financial tasks, respectively, and GPU memory consumption ratio of 6.3X. The sizes of our models are smaller than 0.59 GB, allowing inference on a smartphone.

==> Sections/High_performance_tensor_layer_using_GPU_tensor_cores.tex <==
\section{High-Performance Tensor Computing Using GPU Tensor Cores}
\label{section:High-Performance_Tensor}


\subsection{GPU Tensor Cores for Tensor Computing}
\label{section:tensor_cores}
Modern GPUs have multiple tensor cores to compute matrix multiplications in parallel. The tensor computing consists of multiple independent matrix multiplications. Tensor computing can be accelerated in parallel by GPU tensor cores. For example, the tensor computing process of $\mathcal{G} = \mathcal{G}_2 \circ \mathcal{G}_1, \mathcal{G} \in\mathbb{R}^{r \times n_1 \times n_2 \times r}, \mathcal{G}_1\in\mathbb{R}^{r \times n_1 \times r}, \mathcal{G}_2 \in\mathbb{R}^{r \times n_2 \times r}$ is as follows:
%In Table \ref{table:mm_time}, we show the GPU operation performance and matrix multiplication time at different precisions with $\bm{A}\in\mathbb{R}^{8192\times8192}$ and $\bm{B}\in\mathbb{R}^{8192\times8192}$.

\begin{itemize}
    \item $\mathcal{G}_1$ and $\mathcal{G}_2$ have $r$ horizontal slices and frontal slices, respectively. In tensor computation, these matrices do matrix multiplication with each other.

    \item Each matrix multiplication is mapped to a GPU tensor core. There are $r^2$ matrix multiplications that be computed using $r^2$ tensor cores in parallel.
    % Almost all computations in LLM are matrix multiplications. For example, by using GPU tensor cores, \cite{CP_tensor} achieves up to $30.64\times$ speedup for CP decomposition; \cite{HT_tensor} achieves up to $32.67\times$ speedup for HT decomposition.
    %\item Mixed precision matrix computations using GPU tensor cores are much faster than full precision computation using CUDA cores. Neural networks can be trained with mixed precision without loss of accuracy\cite{micikeviciusmixed}.
\end{itemize}

The number of CUDA cores in A100 GPU is 16$\times$ that of tensor cores. However, The tensor core in A100 GPU executes $256$ multiplication operations per clock, while the CUDA core executes once  \cite{choquette2021nvidia}. When fully utilizing tensor cores, the tensor product is 16 times faster than with cuda cores.

% A100 GPU has $6912$ cuda cores and $432$ tensor cores. Each tensor core executes $256$ multiplication operations per clock \cite{choquette2021nvidia}. that tensor cores accelerate the tensor computation $16 \times $ faster than cuda cores.


%using the pipeline model parallel method as shown in Fig. \ref{fig:pipeline}


\subsection{Quantization of Model Weights and Training Data}
\label{section:quantization}

% \begin{table}
% \caption{The performance at different precisions.}
% \Centering
% \begin{tabular}{ccc}
% \toprule
% Precision & Time (ms) & Performance (TFLOPS)\\
% \midrule
% FP32 & 54 & 19.5\\
% FP16 & 4 & 312\\
% int8 & \textcolor{red}{14} & 624\\
% int4 & - & 1248\\
% \bottomrule
% \end{tabular}
% \label{table:mm_time}
% \end{table}

\begin{table}
\caption{The performance at different precisions.}
\Centering
\begin{tabular}{ccc}
\toprule
Precision & Performance (TFLOPS)\\
\midrule
FP32 & 19.5\\
FP16 & 312\\
int8 & 624\\
int4 & 1248\\
\bottomrule
\end{tabular}
\label{table:mm_time}
\end{table}
% \begin{figure}
% \centering
% \includegraphics[width=9cm]{figs/precision.png}
% \caption{Representative precision support by A100 GPU.}
% \label{fig:precision}
% \end{figure}

The pretrained weights of LLMs typically have the $16$-bit format. However, low-precision data has a smaller size and is better suited for computing using GPU tensor cores as shown in Table \ref{table:mm_time}. Quantization converts data from high-precision to low-precision formats, e.g., int$8$ or int$4$. In this method, we quantize the model weights and training data.
%Quantization represents the pretrained weight $\bm{W}$ as low-precision format, e.g., int8 and int4, which can compress the LLM by $50\%$ and $75\%$. The quantization of weight $\bm{W}$ have three steps as follows:

\textbf{Quantization of Model Weights}

The model weights are in matrix form. We quantize the weights on per-vector. 
The pretrained weight $\bm{W}$ be transferd from CPU memory to GPU memory. In the quantization process, each vector is multiplied by a scaling factor. These multiplications are independent, we batch these vector operations for computation on GPU. 
%\begin{itemize}
    %\item The pretrained weight $\bm{W}$ be transferd from CPU memory to GPU memory. 
    %\item Based on the numerical range, we calculate the quantization scale for each vector.
    %\item $M_i$ is the max value in $i$-th vector of $\bm{W}$. We calculate $\frac{127}{M_i}$ for int$8$ quantization or $\frac{15}{M_i}$ for int$4$ quantization, to obtain the quantization scale of the $i$-th vector.
    %\item Each vector is multiplied by its quantization scale. And then the numerical range of each vector is the numerical range of int$8$ or int$4$ format. We batch these vector operations for computation on GPU. 
    %\item In the quantization process, each vector is multiplied by a quantization scale. These multiplications are independent, we batch these vector operations for computation on GPU. 
%\end{itemize}

\textbf{Quantization of Training Data}

During the training process, the data is sequentially transferred from CPU to GPU. And then we quantize the data on GPU. We quantize the training data into the same data format as the weights. After the quantization, the data and weights are multiplied with low precision. As shown in Table \ref{table:mm_time}, GPUs have better performance in low-precision computations.
% In addition to compressing the model, the low-precision data is also well suited for computation using tensor cores.

% \begin{itemize}
%     \item Low-precision data can fully utilize the computing power of tensor cores.
%     \item Low-precision data has a lower GPU memory footprint, which is important to the training or inference for LLMs on fewer devices.
%     \item Low-precision data has a small size, which can reduce the communication overhead in distributed training.
% \end{itemize}
\begin{figure*}[htbp]
\subfigure[model-parallel]{   %第一张子图
\begin{minipage}{9cm}
\includegraphics[scale=0.17]{figs/model_parallel.png}  %以pic.jpg的0.5倍大小输出
\label{fig:modelparallel}
\end{minipage}
}
\subfigure[pipeline model-parallel]{ %第二张子图
\begin{minipage}{9cm}
\includegraphics[scale=0.17]{figs/pipeline_mdoel_parallel.png}%以pic.jpg的0.5倍大小输出
\label{fig:pipeline}
\end{minipage}
}
\caption{Model-parallel and pipeline model-parallel.}    %大图名称
\label{fig:parallel}    %图片引用标记
\end{figure*}

\subsection{Pipeline Model-Parallel Method for Improving GPU Utilization}
\label{sec:pipeline}

% \begin{figure}
% \centering
% \includegraphics[width=9cm]{figs/pipeline_mdoel_parallel.png}
% \caption{Pipeline model parallelism.}
% \label{fig:pipeline}
% \end{figure}
%The GPU memory footprint for train a large language is much bigger than a single GPU memory capacity. The conventional method use model parallel with multiple GPUs. Different layers of LLM are distributed across these GPUs. During the training, the forward propagation executes serially between these layers of LLM as shown in Fig. \ref{fig:pipeline}. At the same time, only a single GPU is running. These GPUs are severely under-utilization.
%In conventional model parallel, multiple GPUs train an LLM serially with low utilization.
The GPU memory footprint of training LLMs exceeds the capacity of a single GPU, requiring model parallel training methods. However, these GPUs are running serially as shown in Fig. \ref{fig:modelparallel}, resulting in low GPU utilization. In this method, we overlap the computation of multiple GPUs, to improve the GPU utilization.  As shown in Fig. \ref{fig:pipeline}, the training process on four GPUs is as follows:
\begin{enumerate}
\item We split the LLM and transfer it from CPU to $4$ GPUs. Each GPU has a different part of the model.

\item In the forward-propagation, we split the training data into several sub-data, and fed these sub-data into GPU-0 sequentially. On different sub-data, these GPUs can do forward propagation in parallel.

\item The backward-propagation starts with the last GPU. Each GPU calculates the gradient and transfers it to the previous GPU. Similar to forward propagation, the training of each sub-data has a backward-propagation, which can be parallelized across multi-GPUs.

\item Training of each sub-data generates a gradient. We gather these gradients to obtain the final gradient, and then update the LLM.
% The LLM on these four GPUs is do the forward propagation on each parts sequentially.
\end{enumerate}
For training an LLM on $N$ GPUs, the model-parallel as shown in Fig. \ref{fig:modelparallel} has a GPU utilization of $\frac{1}{N}$. With $M$ sub-data, the pipeline model-parallel improves the GPU utilization to $\frac{M}{N+M-1}$.

% Using the pipeline model-parallel, 

%During the training in model-parallel, each GPU stores a part of the model and multiple GPUs collaborate to compute the gradients. As shown in Fig. \ref{fig:pipeline}, the pipeline model-parallel method splits a batch of data into many mini-batches, which are fed sequentially into the model. 

% For training a model on $N$ GPUs, the conventional model-parallel has a GPU utilization of $\frac{1}{N}$. By splitting the batch of data into $M$ mini-batches, model-parallel achieves a GPU utilization of $\frac{M}{N+M-1}$. Take the Llama2-7B model \cite{llama2}  as an example. It has $32$ layers. We train this model on $4$ GPUs with $256$ batch sizes. The forward-propagation for a batch of data is as follows:
% \begin{enumerate}
%     \item We split the Llama2-7B into $4$ parts. Each part has $8$ different layers. Then we load these parts into $4$ GPUs. Similarly, we split the batch of data into $4$ equal mini-batches.
%     \item These $4$ GPUs are running serially on the same mini-batch.
%     \item After running on a mini-batch, the GPU transfer the outputs to the next GPU and load the next mini-batch. On different mini-batches, these $4$ GPUs can be running in parallel.
% \end{enumerate}
% The backward propagation is similar to forward propagation. It starts from the last GPU and calculates the gradients of each mini-batch. The gradients of these mini-batches are accumulated as the final gradients, which are equal to the gradients of the whole batch.

%By scheduling the forward-propagation and back-propagation of training on multiple GPUs, model parallelism can reduce the memory footprint of intermediate outputs. We know that the size of intermediate outputs is correlated with the batch size and the intermediate outputs be freed after back-propagation. 

% \begin{enumerate}
%     \item We split the LLaMA-7B into $4$ sub-models. Each sub-model has $8$ different layers. Then we transfer these sub-models from CPU to $4$ GPUs, e.g. GPU$_0$ has the $1$th $\sim$ $8$th layers, GPU$_1$ has $9$th $\sim$ $16$th layers, ..., GPU$_4$ has the $24$th $\sim$ $32$th layers.
%     \item The input has $256$ batch sizes. We split it into $4$ sub-inputs. Each sub-input has $64$ mini-batch sizes. We get the input$_0$, input$_1$, input$_2$ and input$_3$.
%     \item We transfer the input$_i$ from CPU to GPU-0. The input$_i$ is fed into the sub-model$_0$ and generated the output, with $i = 0,1,2,3$. Then we transfer the output from GPU$_0$ to GPU$_1$
%     \item When GPU$_j$ get the output$_i$ from GPU$_{j-1}$, we feed it into sub-model$_j$ and obtain the new output$_i$. Then we transfer the new output$_i$ from GPU$_j$ to GPU$_{j+1}$, with $j=1,2$.
%     \item GPU$_4$ get the output$_i$ from GPU$_3$. We feed it into sub-model$4$ and get output$_i$, with $i = 0,1,2,3$. Gathering these outputs, we get the final output.
% \end{enumerate}



%Taking the A100 GPU as an example, it has $432$ tensor cores. Each tensor core can execute a product with two matrices per clock with mixed precision, that two matrices have the size of $8 \times 4$ and $4 \times 8$. This means that a tensor core can perform 256 fused multiply-add operations at once.

%For a matrix multiplication $\bm{C} = \bm{A}\bm{B}$ with $\bm{A} \in \mathbb{R}^{32\times32},\bm{B} \in \mathbb{R}^{32\times32}$ and $\bm{C} \in \mathbb{R}^{32\times32}$, 

% tensor computing

\subsection{Reducing Memory Footprint of Intermediate Variables}
\label{sec:inter_out_rec}
Intermediate variables have a huge memory footprint during the training. We show the GPU memory footprint of training Llama2-70B in Fig. \ref{fig:GPUmemoryforllama}. With batch size=$1$, the intermediate variables have a GPU memory footprint of $485$ GB. And the memory footprint of the intermediate outputs increases with batch size, contributing to most of the huge memory footprint. 

By avoiding the storage of intermediate variables and recomputing them when needed, the GPU memory footprint can be significantly reduced, at the cost of an increased computation. Intermediate variables are generated in forward propagation, used in backward propagation, and then released. 
%However, intermediate results are used in the reverse order of generation
%The outputs of linear layers, activation functions, dropout layers, etc, need to be stored to calculate gradients, resulting in a large memory footprint. 
In this method, Only the input data for each layer is stored in the GPU memory. In back-propagation, the GPU recomputes intermediate variables of each layer using the input data. For each layer in LLMs, the memory footprint of intermediate variables is hundreds of times larger than the memory footprint of input data. And the computational workload for recomputing intermediate variables is the same as for forward propagation. The GPU memory footprint of intermediate variables can be reduced by $99\%$ with a $33\%$ increase in computation.

By selectively recomputing the intermediate outputs, there is a good balance between memory consumption and computation. Some intermediate outputs have a large memory footprint but required a slight computation. For example, training an LLM with sequence length=$n$, the low-rank tensor layers and matrix multiplication $QK^{T}$ have the same output size. However, the computation of the matrix multiplication is $n$ times that of low-rank tensor layers. By recomputing modules with large output sizes but low computational cost, the memory footprint of training LLM can be reduced by about $90\%$, with a $5\%$ increase in computation as a trade-off.


\begin{figure}[t]
\centering
\includegraphics[width=9cm]{figs/cpu-gpu_memory.png}
\caption{Virtural GPU memory.}
\label{fig:vgpumemory}
\end{figure}


%(It is important to tensor layer-based LLMs. The low-rank tensor layers can reduce the number of parameters in LLMs, but not for intermediate outputs. The low-rank tensor layers have the same size of outputs with the $\bm{W} \in \mathbb{R}^{n \times m}$, and some intermediate values which has the same size of rank.)
\subsection{Reducing Memory Footprint of Optimizer States}
\label{section:mem_and_opt}
Except for intermediate results, the optimizer states consume most GPU memory footprint during the training, as shown in Fig. \ref{fig:GPUmemoryforllama}. The data in GPU memory can be classified into two main categories as follows:
\begin{itemize}
    \item \textbf{Parameters and Gradients.} In mixed-precision training, model parameters and gradients have the same size and are in $16$-bit data format.
    \item \textbf{Optimizer States.} Most training of LLMs use the AdamW optimizer \cite{adamw}. It contains the full-precision parameters and two states, momentum and variance, each state has the same size as the model.
\end{itemize}
\label{sec:opt_sta}
As shown in Fig. \ref{fig:GPUmemoryforllama}, during the training of Llama2-70B, these data have a total of $1,120$ GB of GPU memory footprint, of which the optimizer states account for about $840$ GB.

\textbf{Split the Optimizer States}

Optimizer states and gradients can be split into multiple GPUs to reduce GPU memory footprint during the training. In conventional data parallelism, each GPU stores complete parameters, gradients, and optimizer states. In each iteration, these GPUs communicate their gradients to obtain a global gradient, which they use to update their parameters by the optimizer. We know that optimizer states and gradients correspond to parameters. When training with data parallelism using $N$ GPUs, the optimizer states and gradients can be split into $N$ parts. The training has four steps as follows:
\begin{itemize}
    \item Each GPU has the complete parameters and $i$-th part of optimizer states and gradients, with $i=1,,,,N$.
    \item During the back-propagation, the $i$-th GPU retain only the $i$-th part of gradients. The other gradients be communicated with the corresponding GPU and discarded.
    \item The $i$-th GPU gather the $i$-th part of gradients, and obtain the $i$-th part of new parameters by optimizer.
    \item Each GPU communicates its new parameters to others. All GPUs obtain completely new parameters.
\end{itemize}
Using $8$ GPUs to train an LLM with $70$B parameters, the memory footprint be reduced from $1120$ GB to $262.5$ GB.


\textbf{Virtural Memory for Optimizer State.}

By exploiting CPU memory storage optimizer states, the peak GPU memory footprint is reduced. Optimizer states are not required in the forward and backward propagation stages. In these two stages, the optimizer states can be transferred to CPU memory, like virtual memory. In the weight update stage, the intermediate outputs be freed, and the optimizer states are transferred back into GPU memory as shown in Fig. \ref{fig:vgpumemory}. 





==> Sections/tensor_layer_for_large_image_datasets.tex <==

\section{Application to Large Image Datasets}
\label{section:tl_image}

\subsection{Challenges of Large Image Datasets}
% ImageNet-1K and ImageNet-21K
Training a deep neural network on large-scale image datasets is highly computing-intensive. Many researchers use data parallelism to train their models on distributed servers. Data parallelism based on distributed stochastic gradient descent (SGD) utilizes the parameter-server architecture \cite{li2014communication}. We show the training process as in Fig. \ref{fig:paralleltraining}. 

There are several major challenges:
\begin{itemize}
    \item For each iteration, these nodes need to transfer the model and gradient, incurring large communication overhead.
    \item The workload of each node is imbalanced. The communication overhead of the master server is equal to the sum of other nodes' overhead.
    \item When the master server fails, the whole training process will be interrupted. When a worker server fails, the training process will be delayed.
\end{itemize}

\subsection{Motivating Example}
\label{motivating_example}

\textbf{IDEA}: The circular convolution in the time domain corresponds to element-wise multiplication in the spectral domain. In the spectral domain, the t-product can be separated into multiple independent matrix products, as shown in Fig. \ref{fig:t-product_in_spectral}, that possess strong parallelism \cite{zhang2019cutensor}.

We use the MNIST\cite{deng2012mnist} dataset as an example. This is a large collection of handwritten digits, where each sample is a grey image. The training process consists of the following two steps:
\begin{itemize}
    %\item \textbf{Data splitting}: In this dataset, each image $\bm{X}$ has size of $28 \times 28$. For split it into 16 subs, we sample every $4$ steps on mode-1 tubes and every $4$ steps on mode-2 tubes, then combine these $\frac{28}{4}\times\frac{28}{4}$ pixels to get a new sub image $\bm{X}_q \in \mathbb{R}^{7 \times 7}, q \in [1,...,16]$. Concatenating this sub images, the input be represented as $\mathcal{X} \in \mathbb{R}^{7 \times 7 \times 16}$. By doing $\mathcal{L}$ along the last dimension, we have $\mathcal{X}$ in spectral domain $\hat{\mathcal{X}} \in \mathbb{R}^{7 \times 7 \times 16}$. Spliting $\hat{\mathcal{X}}$ along the last dimension, we have $16$ sub images in the spectral domain. Spliting all images in the dataset, we have $16$ independent sub-datasets in spectral domain.

    \item \textbf{Data splitting}: In this dataset, each image $\bm{X}$ has size of $28 \times 28$. We downsample the image by stride = $4$ to get 16 new images $\bm{X}_q \in \mathbb{R}^{7 \times 7}, q = 1, 2, ..., 16$. Concatenating this images, the input be represented as $\mathcal{X} \in \mathbb{R}^{7 \times 7 \times 16}$. By doing $\mathcal{L}$ and splitting $\mathcal{X}$ along its last dimension, we have $16$ sub-images in the spectral domain. Splitting all images in the dataset, we have $16$ independent sub-datasets in the spectral domain.
        
    \item \textbf{Parallel training}: We split the network into $16$ sub-networks. The $q$-th sub-network training on the $q$-th sub-dataset, $q = 1, 2, ..., 16$. These training processes are asynchronous and independent, there is no communication with each other.
\end{itemize}

In the inference process, we split the validation image into $16$ inputs in spectral domain. The $q$-th sub-network inference on $q$-th input, generating $q$-th result, $q = 1, 2, ..., 16$. Weighted summing these results, we obtain the final result.
Take a sample in MNIST dataset \cite{deng2012mnist}, the data-splitting as shown in Fig. \ref{fig:mnist_split}.


% \begin{itemize}
%     \item \textbf{Data spliting}: Image input $\mathcal{X}$ has size of $H \times W \times C$. $C = 1$ on grey image and $C = 3$ on colour image. We sample every $q_1$ steps on mode-1 tubes and every $q_2$ steps on mode-2 tubes, then combine them to get a new sub image $\mathcal{X}_q \in \mathbb{R}^{\frac{H}{q_1} \times \frac{W}{q_2} \times C}, q \in [1,...,Q]$. Concatenating this sub images, the input be represented as $\mathcal{X} \in \mathbb{R}^{\frac{H}{q_1} \times \frac{W}{q_2} \times C \times Q}$. By doing $\mathcal{L}$ along the last dimension, we have $\mathcal{X}$ in spectral domain $\hat{\mathcal{X}} \in \mathbb{R}^{\frac{H}{q_1} \times \frac{W}{q_2} \times C \times Q}$. Spliting $\hat{\mathcal{X}}$ along the last dimension, we have $Q$ sub iamges with $Q = q_1 \times q_2$. Spliting all images in a dataset, we have $Q$ independent sub-datasets.
        
%     \item \textbf{Parallel training}: We split the network into $Q$ sub-networks. The $q$-th sub-network training on the $q$-th sub-dataset, $q \in [1,Q]$. These  training processes are asynchronous and independent, there is no communication with each other.
        
%     \item \textbf{Ensemble learning}: In inference procedures, we split the validation images into $Q$ sub-images. $q$-th sub-network inference on $q$-th sub-image, generating $q$-th result, $q \in [1,Q]$. Weighted sum these results, we obtain the final result.
    
% \end{itemize}

%Using the MNIST \cite{deng2012mnist} dataset as example, the data spliting as shown in Fig. \ref{fig:mnist_split}. This is a large collection of handwritten digits. It has $60,000$ training images and $10,000$ testing images. Each image has a size of $28 \times 28$. Taking a sample $X \in \mathbb{R}^{28 \times 28}$, we have input $\mathcal{X} \in \mathbb{R}^{7 \times 7 \times 16}$ after downsample for stride $q_1 = q_2 = 4$. Doing transform on the mode-3 tubes of $\mathcal{X}$, we have $16$ sub-images. 
\begin{figure*}[t]
    \centering
    \includegraphics[width=18cm,height=6cm]{figs/mnist_split.png}
    \caption{Splitting a sample in MNIST dataset.}
    \label{fig:mnist_split}
\end{figure*}

\subsection{Training of Parallel Branches}

Distributed training on large-scale datasets has a large communication overhead. The image count of large-scale datasets can reach tens of millions. Conventional distributed training using the parameter-server architecture as shown in Fig.$\ref{fig:paralleltraining}$. In an iteration
%, the master node distributes the model to other slave nodes. Each node trains the model on its own batch of data, and the slave nodes send grads to the master node. 
the communication overhead of each slave node is twice the model size, and 
the communication overhead of the master node is the sum of the other slave nodes. Scaling distributed nodes leads to increasingly complex communications, which in turn reduces the benefits of distributed training. For example, compared to training ResNet34 with a single GPU, using $2$ GPUs achieved a speedup of $1.93\times$, and using $6$ GPUs achieved a speedup of only $4.07 \times$.

By spectral tensor layer, We implement a distributed training strategy without communication overheads. 1) The training dataset be split into some sub-dataset in the spectral domain as shown in Section \ref{motivating_example}. Splitting a dataset into $n$ sub-datasets, the image size is reduced to $\frac{1}{n}$ of the original image size. And these sub-datasets are sent to $n$ computing nodes. 2) In the training stage, we first initiate $n$ sub-networks, mapping each network to a computing node. These networks are trained on different spectral sub-datasets, Instead of communicating gradients, they learn different features
in the spectral domain.
For input $\bm{x} \in \mathbb{R}^{n^2}$, the size of linear layer is $n^4$, as in Table \ref{table:s_t_diff_method}. In sub-datasets, the size of input $\bm{x}$ be reduced from $n^2$ to $n$, that the size and multiplication of linear layers be reduced from $n^4$ to $n^2$.
% For example, training the ResNet50\cite{he2016deep} on ImageNet-21K\cite{deng2009imagenet} dataset with $8$ nodes, The communication overheads of the master and slave nodes are $3.6$ GB and $0.5$ GB in each iteration. 





==> Sections/tensor_layer_in_llm.tex <==
\section{Application to Large language Models}
\label{section:tl_in_llm}

\subsection{Challenges of Large Language Models}
\label{challenges_llm}

%Large language models have a large number of parameters, which means a large amount of computation. And in order to give the large language model strong generalization abilities, it requires a large scale of training data. Taking LLaMA-65B \cite{touvron2023llama} as an example, to train this model used dataset with $4.7$TB. The large-scale dataset also means the long training time. In Table \ref{table:llama}, we show the number of paramteres and training time for some large language models.


% 大语言模型的训练时间、存储空间

% \textbf{Method 1}: pmap for decomposing; vmap for fine-tuning.

% \textbf{Method 2}: vmap fro train-from-scratch

% \textbf{Method 3}: \textbf{Quantized tensor layer} (similar to QLoRA)

%Most large language models are based on the transformer architecture \cite{vaswani2017attention}, as shown in Fig. \ref{fig:transformer}. There contains many linear layers as in (\ref{eq:linear_layer}), which is particularly applicable to the tensor layer method. We have the following three methods:

\begin{figure}[t]
\centering
\includegraphics[width=9cm]{figs/flowoflora.png}
\caption{Flow of method 1.}
\label{fig:flowofmethod1}
\end{figure}

\subsection{Method 1: Low-rank Adaption (LoRA)}
\label{sec:lora}

Several organizations have released foundation LLMs\cite{touvron2023llama} \cite{scao2022bloom}\cite{falcon}. Many companies intend to have domain-specific LLMs based on these foundation LLMs. Bloomberg has launched BloombergGPT \cite{wu2023bloomberggpt}, a financial domain LLM. In financial tasks, BloombergGPT is reported to have better results than many general LLMs, e.g., OPT-$66$B \cite{zhang2022opt}, BLOOM-176B\cite{scao2022bloom}, and it has a training cost of \$3.2 million. 

\textbf{Method}: Low-rank adaptation (LoRA) method \cite{hulora} provides a low-cost fine-tuning solution for LLMs. This method fine-tunes a pretrained LLM on the domain-specific dataset. The fine-tuned LLM has knowledge of the specific domain. Given a pretrained LLM with weight $\bm{W}$, the LoRA method adapts it to  $\bm{W}^{'} = \bm{W} + \Delta \bm{W}$ by adding a low-rank $\Delta\bm{W} = \bm{B} \bm{A}$. The idea of the LoRA method \cite{hulora} is as follows:
\begin{equation}
\label{eq:new_linear_layer}
\bm{W}^{'}\bm{x} =(\bm{W}+\Delta\bm{W})\bm{x}= \bm{W}\bm{x}+\bm{B}\bm{A}\bm{x},
\end{equation}
During the training stage, we freeze the weight $\bm{W}$ and train the low-rank factors, $\bm{B}$ and $\bm{A}$. In the inference stage, the $\bm{B}\bm{A}$ is added to $\bm{W}$ and we use $\bm{W}'$.
%Given a new domain-specific dataset, the low-rank adaptation (LoRA) method \cite{hulora} was proposed as a lightweight adaptation of an LLM to a new industry.

%Many industries want to use them to get their own domain-specific LLMs for online services. Bloomberg has launched BloombergGPT \cite{wu2023bloomberggpt}, which is a financial domain LLM, and has a training cost of \$3.2 million. 

%Since LLMs are trained at a huge cost, it is expected to scale it to hundreds of industries (different application scenarios) at a low adaptation cost. Given a new domain-specific dataset, the low-rank adaptation (LoRA) method  \cite{hulora} was proposed as a lightweight adaptation of a LLM to a new industry.

%The multi-head attention layer has $n$ attention modules. The layer concatenate this attention modules output and product with $\bm{W}^O$. The attention module has three inputs, $K, Q, V$. This input do product with weight matrix $\bm{W}_i^K, \bm{W}_i^Q, \bm{W}_i^V, i \in [1,n]$, respectively, before
%Inputting them into attention module. This weight $\bm{W}_i^K \in \mathbb{R}^{d_{in} \times d_{out}}, \bm{W}_i^Q \in \mathbb{R}^{d_{in} \times d_{out}}, \bm{W}_i^V \in \mathbb{R}^{d_{in} \times d_{out}},$ and $\bm{W}^O \in \mathbb{R}^{d_{in} \times nd_{out}}$, $d_{in} = n \times d_{out}$. 

%The feed-forward module is two fully connected layers which can be represented as follows:
%where $\sigma(\cdot)$ is activation function, $ \bm{W}_1 \in \mathbb{R}^{d_{in} \times 4d_{in}}$, $\bm{W}_2 \in \mathbb{R}^{4d_{in} \times d_{in}}$ is weight matrix, $ \bm{b}_1 \in \mathbb{R}^{4d_{in}}$, $\bm{b}_2 \in \mathbb{R}^{d_{in}}$ is bias vector.

%The multi-head attention module has $4d_{in}^2 = d_{in} \times d_{out} \times 3 \times n + d_{in} \times nd_{out}$ parameters, and feed forward module has $8d_{in}^2 = d_{in} \times 4d_{in} \times 2$ parameters without bias vector.

%Fine-tuning the large language model make the weight $\b{m}$ transfer from $\bm{W}_{old}$ to $\bm{W}_{new}$. In essence, this is about learning a $\Delta \bm{W} = \bm{W}_{new} - \bm{W}_{old}$. The new linear layer can be represented as follows: 

%The $\Delta\bm{W}$ also can be represented as tensor layers as in Section \ref{sec:tensor_layer}. 

We map the above method onto GPU as follows:

% \textbf{forward} Individuals want to fine-tune an LLM on a single GPU. The LoRA method still consumes a large amount of GPU memory, which exceeds the capacity of a single GPU. By analyzing (\ref{eq:new_linear_layer}), we know that the GPU memory consumption can be classified into four parts: 1) the pretrained weight $\bm{W}$; 2) the trainable low-rank layer $\bm{A}$ and $\bm{B}$; 3) the input data $\bm{x}$ 4) the intermediate variables in forward propagation.
%the input data $\bm{x}$; and the intermediate variables at different layers, which is the result of $\bm{W}\bm{x}+\bm{B}\bm{A}\bm{x} $ in $(\ref{eq:new_linear_layer})$.

\textbf{Quantize}: Low-rank adaptation method significantly reduces the number of trainable parameters. However, pretrained weights have a larger memory footprint. For example, the pretrained weights of Llama2\cite{llama2} consume $140$ GB GPU memory during the fine-tuning. In our method, the pretrained weights are quantized to low precision. 
\begin{itemize}
    \item The pretrained weight $\bm{W} \in \mathbb{R}^{n \times n}$ has $n$ vector, calculating the difference between the maximum and minimum values to get the scaling factor of each vector.
    \item In each vector, there are $n$ elements multiplied with scaling factor. These multiplications are batched by mapping on $n$ CUDA cores.
    \item Results are stored in low-precision formats, such as int8 or int4, in GPU memory, while the original weights are deleted.
\end{itemize}
% Depending on the accuracy required, the data format of weights can be quantized to 8bit or 4bit.
Using the quantization, the GPU memory footprint of pretrained weights can be reduced from $140$ GB to $70$ GB by and $35$ GB, respectively.

\textbf{Forward}: As shown in Table \ref{table:llm_pandt}, the training data for LLM has a large size. It is stored in the disk and transferred into the GPU memory while training. However, compared to CPU and GPU memory, disk has low bandwidth and high latency. In our method, the training data is prefetched from disk to CPU memory. The training process is as follows:
\begin{itemize}
    \item While the GPU is working, multiple CPU threads load data from the disk into CPU memory. One thread transfers data from CPU memory to GPU memory, when GPU requires input data $\bm{x}$.
    \item Quantizing $\bm{x}$ as $\hat{\bm{x}}$, $\hat{\bm{x}}$ do the matrix multiplied with the quantized weight $\bm{W}$ using tensor cores. The output is batched dequantize to $\bm{y_1}$.
    \item $\bm{x}$ do the tensor product with the low-rank tensor layer using tensor cores, to get the output $\bm{y_2}$
    \item $\bm{y_1}$ and $\bm{y_2}$ are added to obtain $\bm{y}$, which is the input data for the next layers. It is deleted with other intermediate variables after calculating from GPU memory. 
\end{itemize}

% Based on the input data, the fine-tuning process generates a large number of intermediate variables. 
For fine-tuning a $7$B LLM, the GPU memory footprint of intermediate variables exceeds the memory capacity of one A100 GPU. 
%The input data is quantized into the data format of weights for computing. The intermediate variables are in low-precision format. And 
We do not store the most intermediate variables in the GPU memory, only the input of each decoder layer. That can reduce the memory consumption of intermediate variables by more than $90\%$.
%recomputing them in the back-propagation as in Section \ref{sec:inter_out_rec}. 

\textbf{Backward}: In backward propagation, the model uses the intermediate variables to compute the gradients of parameters. However, intermediate variables are not stored. In this method, We use the recomputing method as in Section \ref{sec:inter_out_rec}. 
\begin{itemize}
    \item In the backward propagation of each decoder layer, GPU first computes as the forward to obtain intermediate variables.
    \item Using intermediate variables and parameters, the GPU calculates the gradients of low-rank layers, which are updated depending on the gradient and optimizer states.
\end{itemize}
  Only the low-rank layers have the trainable parameters, which can significantly reduce the memory footprint of the gradients and optimizer states. Compared to the low-rank matrix layers $\bm{A}$ and $\bm{B}$, low-rank tensor layers are more compact, as given in Table \ref{table:s_t_diff_method}. During the fine-tuning of Llama2, the low-rank tensor layers reduce the memory footprint of the gradients and optimizer states from 840 GB to about 1 GB.

%intermediate variables in low-rank layer $\bm{A}$ and $\bm{B}$ have fewer parameters than weight $\bm{W}$. However, the fine-tuning produces gradients and optimizer states for trainable weights, as shown in Section \ref{section:mem_and_opt}. Our method uses the low-rank tensor layer instead of the low-rank matrix layer.  To match the tensor production, we matrixize input data $\bm{x}$ before feeding into the low-rank tensor layer. And the output of low-rank tensor layers is vectorized to sum with the output of the frozen weight $\bm{W}$. During the fine-tuning of Llama2, the low-rank tensor layer can reduce the GPU memory footprint of $\bm{A}$ and $\bm{B}$ from $702$ MB to $21$ MB.
%By tensorizing the data into high dimensions, we represent $\Delta\bm{W}$ as low-rank tensor layers.

\textbf{Inference} During the fine-tuning, low-rank layers increase the total number of parameters in LLMs. These parameters can be merged with the original parameters. For the low-rank layer of weight $\bm{W} \in \mathbb{R}^{n \times n}$, there are some tensor factors. These tensor factors are contracted to a tensor $\mathcal{W}_t$ using GPU tensor cores. Matrixing $\mathcal{W}_t$ to $\bm{W}_t$, $\bm{W}_t$ have the same size as weight $\bm{W}$. Adding $\bm{W}$ and $\bm{W}_t$ to obtain $\bm{W}^{'}$, $\bm{W}^{'}$ is the new weight.

% The training dataset of LLMs has a large scale, posing significant storage and computational challenges. 1) As in Sec. \ref{section:train_from_scratch}, The data is loaded from the disk into CPU memory in batches and then transferred to the GPU memory for training. 2) For multi-GPU servers, different batches of data in CPU memory are transferred to different GPUs for parallel training. 

%The memory consumption of intermediate variables is more than half of training LLMs. We quantize the input data to match the data format of $\bm{W}$. The low-precision outputs have a lower GPU memory footprint. 
%By quantizing $\bm{W}$ into int$8$ and int$4$ as in Section \ref{section:quantization}, the memory footprint of pre-trained weights is reduced from $13.8$ GB to $8.1$ GB and $4.8$ GB. And during the fine-tuning, the input $x$ is quantized to match the data format of $\bm{W}$. After quantization, we have reduced the GPU memory footprint from $34$ GB to $10.6$ GB. The frozen linear layers have much more computations than low-rank layers as given in Table \ref{table:s_t_diff_method}. The matrix multiplication of quantized $\bm{W}$ and $\bm{x}$ is more suitable for GPU tensor cores in (\ref{eq:new_linear_layer}) as in Section \ref{section:tensor_cores}.

%Weights $\bm{W}$ and inputs $\bm{x}$ have the most GPU memory footprint. During the fine-tuning, there is a GPU memory footprint of $34$ GB. Low-rank layers $\bm{A}$ and $\bm{B}$ have a small memory footprint, less than $100$ MB, while pretrained weights $\bm{W}$ have a GPU memory footprint of $13.8$ GB. And inputs $\bm{x}$ have a memory footprint of $19.3$ GB (batchsize=$8$).


%%%%%%下面内容填充到四段话里%%%%%%%%%%


%Fine-tuning with the low-rank layers has a $34$ GB memory footprint. However, it is still a challenge for many GPUs. When training an LLM, four types of data have the most GPU memory footprint:

% \begin{itemize}
%     \item \textbf{Parameters.} In mixed-precision training, the model parameters are updated in full precision ($32$-bit) and calculated in half-precision ($16$-bit), which has $4+2$ bytes GPU memory overhead.
%     \item \textbf{Gradients.} In training, the back-propagation generates gradients, which have the same size as half-precision model parameters.
%     \item \textbf{Optimizer States.} Most training of LLMs use the AdamW optimizer \cite{adamw}. It has two optimizer states, each has the same size with the full-precision model.
%     \item \textbf{Intermediate Outputs.} The size of intermediate outputs is related to the batch size of input and dimension size of the model. 
% \end{itemize}
%During the training with LoRA method, parameters contain frozen pertaining parameters and trainable parameters, which have memory footprint of $13.8$ GB and $16$ MB respectively. Due to the few trainable parameters, gradients and optimizer states have less than $1$ GB of GPU memory footprint.


%Low-rank matrices $\mathbf{A}$ and $\mathbf{B}$ have much fewer parameters than the pretrained weights $\mathbf{W}$. For example, there are $4.2$ million of trainable parameters when we finetune the LLaMA-7B model with $6.7$ billion of parameters. These frozen pretrained weights and trainable parameters have a GPU memory footprint of $13.4$ GB + $67.2$ MB.


%Weight $\mathbf{W}$ are quantified vector-wise \cite{llmint8}. Quantizing weight $\mathbf{W} \in \mathbb{R}^{n \times n}$ have a parallelism of $n$. During the training, the inverse quantization has the same parallelism. We batch these quantization and de-quantization operations for computation on the GPU.


% \begin{algorithm}[t]
% \caption{Quantization and de-quantization} 
% \label{quan}
% \begin{algorithmic}[1]
% \STATE \textbf {Quantization}: 
% \STATE \textbf{Input}: High-precision weight $\mathbf{W}^{high} \in \mathbb{R}^{n \times n}$.
% \STATE for $i=1$ to $n$ do in parallel : 
% \STATE ~~~~$\mathbf{W}^{low}(i,:) $ = quantization($\mathbf{W}^{high}(i,:)$),
% \STATE \textbf{Output}: Quantified weight $\mathbf{W}^{low} \in \mathbb{R}^{n \times n}$.
% \STATE
% \STATE \textbf {De-quantization}: 
% \STATE \textbf{Input}: Quantified weight $\mathbf{W}^{low} \in \mathbb{R}^{n \times n}$, bias $b \in \mathbb{R}^{n}$ model input  $\mathbf{X} \in \mathbb{R}^{b \times n}$
% \STATE for $i=1$ to $n$ do in parallel : 
% \STATE ~~~~$\mathbf{W}^{high}(i,:) $ = quantization($\mathbf{W}^{low}(i,:)$),
% \STATE$\mathbf{Y}$=$\mathbf{W}^{high}\mathbf{X} + \bm{b}$,
% \STATE \textbf{Output}: $\mathbf{Y}$.
% \end{algorithmic}
% \end{algorithm}

%During the training, the pretrained weight has the GPU memory footprint of $13.4$ GB, and the trainable parameters in low-rank layers has the GPU memory footprint of $67.2$ MB.

 %Two-dimensional low-rank matrices reduce the GPU memory footprint associated with parameters (parameters, gradients, and optimizer stats), not intermediate outputs. The output vector of linear layers with $\mathbf{W} \in \mathbb{R}^{n^2\times n^2}$ has the size of $n^2$, while the low-rank matrix layers with $\mathbf{A} \in \mathbb{R}^{r\times n^2}$ and $\mathbf{B} \in \mathbb{R}^{n^2\times r}$ have two output vectors, that have size of $r$ and $n^2$. 
 
%Compared to the low-rank matrix layers, low-rank tensor layers are more compact, as given in Table \ref{table:s_t_diff_method}. By tensorizing the data into high dimensions, the low-rank tensor layers have much fewer parameters than low-rank matrix layers. By representing $\Delta\bm{W}$ as low-rank tensor layers in Section \ref{sec:tensor_layer}, the GPU memory footprint can be further reduced. 

%It reduces the memory foorprint of the frozen weights by $50\%$ and $75\%$. For example, When fine-tuning LLaMA-65B, the memory footprint can be reduced by $65$ GB and $97.5$ GB for $8$-bit quantification and $4$-bit quantification. 


%During the fine-tuning, the pretrained weight is frozen. We can quantify the pretrained weight $\bm{W}$ from 16-bit to 8-bit or 4-bit. For example, the LLaMA-

%In Section \ref{sec:tensor_layer}, we show the tucker and tensor train decomposition methods. Compare to low-rank matrices, these methods have a higher compression ratio.

%Considering that $\bm{W} \in \mathbb{R}^{4,096 \times 4,096}$ accounts for $99.98\%$ in the linear layer, this method can achieve a compression rate of $99.59\%$, $99.94\%$ and $99.93\%$, respectively.

%We can fine-tuning all or some weight $\bm{W}$ in multi-head attention and feed forward module.

%The input of the multi-head attention is replicated into $3$ parts, $K, Q, V$. Inputting them into attention module after they product with weight matrix $W_i^K, W_i^Q, W_i^V, i \in [1,n]$, respectively.

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=16cm,height=8cm]{figs/paralleltraining.png}
%     \caption{The training process using distributed SGD.}
%     \label{fig:paralleltraining}
% \end{figure*}

\subsection{Method 2: Decomposing-and-Fine-Tuning}
\label{section:two_stage}

Individuals may want to take advantage of the available open-source LLMs and obtain a customized LLM. However, in Section \ref{sec:lora}, the fine-tuned LLM has the same size as the original model, which has a high inference cost. We know that pretrained models have a very low intrinsic dimension, and larger models tend to
have lower intrinsic dimensions \cite{aghajanyan2021intrinsic}. We propose to decompose the linear layers' weights of an open-sourced LLM, using those weights to initialize a tensor layer-based LLM. Therefore, we are motivated to investigate \textit{\textbf{how much speedup can be obtained by using a pretrained LLM to initialize a tensor layer-based LLM?}}

Our method has two stages as follows:
\begin{itemize}
    \item Given the weight of a pretrained LLM, we decompose the weight $\bm{W}$ in linear layers to low-rank tensor layers.  After decomposition, we obtain a tensor layer-based LLM, whose accuracy is lower than the pretrained LLM, as the case in \cite{yong2016compression}.
    \item Then, we fine-tune the tensor layer-based LLM by feeding data (original data and new private data) to improve the accuracy.
\end{itemize}

\textbf{Tensor decomposing in parallel}

Decomposing weight $\bm{W}$ at different linear layers is independent. For example, Llama2-70B has $80$ decoder layers, and each decoder layer has $7$ linear layers. The decomposition stage has a parallelism of $560$. In this method, we distribute decoder layers in an LLM evenly across multiple GPUs. For an LLM that has $n$ linear layers in a decoder layer, the $i$-th linear layers in different decoder layers have the same size, $i = 1,...,n $. In a single GPU, we batch the decomposition of $i$-th linear layer in different decoder layers. On different GPUs, we perform the decomposition in parallel.

%For an LLM with $N$ decoder layers and $M$ GPUs, each GPU has $\frac{N}{M}$ decoder. 

After the decomposition, we fine-tune the low-rank tensor-based LLM with full parameters. The full-parameter fine-tuning can be viewed as pretraining where the model is specially initialized. We use the same method as in Sec. \ref{section:train_from_scratch} for fine-tuning. 

The fine-tuned low-rank model has approximate or even better performance\cite{yin2021towards} and a much smaller model size\cite{HT_tensor}. The device requirement has significantly reduced during the inference. For example, decomposing the linear layers into low-rank matrix layers, the number of parameters in Llama2 reduced from $70$B to $3$B, which consumes $7$ GB GPU memory footprint during the inference.
% \textbf{bottleneck}: the computation cost for decomposition.

% \textbf{tricks}: Decomposing weight $\bm{W}$ at different linear layers is independent.

% The low-rank model with decomposed pretrained weights can recover accuracy by training on a small amount of data. Compared to method-1 in Section \ref{section:train_from_scratch}, This method reduces the training time over 10$\times$.

%For a large language model which has $N$ linear layers. The parallelism of decomposition is $N$. A large language model is transferred to multiple GPUs for training. Each GPU has different layers of the model. We use the Pamp to parallelize the decomposition across different GPUs and use the Vmap to parallelize the decomposition in a signal GPU.

%After decomposing, The fine-tuning process is using the pipeline model parallel as in Section \ref{section:train_from_scratch}.

%We load and transfer the pretrained model from CPU to GPUs. Each GPU has some sublayers. The weight $\bm{W}$ is decomposed into tensor layers in Section \ref{sec:tensor_layer}. For $N$ linear layer in a model, the decomposition process has a parallelism of $N$. We use the pamp to parallelize the decomposition across different GPUs, and use the vpmap to parallelize the decomposition in a signal GPU.

%After decomposing, we fine-tune the model using the pipeline model parallelism.

%After being decomposed, the model's performance may significantly decrease. However, the model can be recovered with fine-tuning \cite{yong2016compression}. 
%(Reducing model size)

%A two-stage method for compressing, and deploying on mobile devices.


\subsection{Method 3: Pre-training LLMs Using Tensor Layers}
\label{section:train_from_scratch}

% \begin{figure}[t]
% \centering
% \includegraphics[width=8cm]{figs/transformer.png}
% \caption{The transformer architecture.}
% \label{fig:transformer}
% \end{figure}

Pre-training weights are required in Section \ref{sec:lora} and Section \ref{section:two_stage}. We aim to provide an economic way for many institutes to pre-train LLMs. However, existing LLMs in Table \ref{table:llm_pandt} incur high pre-training costs, e.g., the computing cost maybe from $\$5$M\cite{zhang2022opt} to even $\$10$M \cite{scao2022bloom}.

%Low-rank tensor layers can significantly reduce the training time of deep neural networks \cite{CP_tensor}. Compared to a full-rank model with the same configuration, the low-rank LLM has a very much smaller number of parameters. Before starting a pretraining of LLM with a huge number of parameters, the low-rank model can be used as a validation of the training settings. Low-rank tensors can be contracted into full-rank tensors to make a full-rank LLM. Pre-training can be based on this model when the correct settings are obtained.

% with little accuracy loss. Because the intrinsic dimension of a deep neural network is much lower than the direct parameter dimension \cite{limeasuring}, while low-rank tensor layers are more compact than the linear layer \cite{liu2022book}, as given in Table \ref{table:s_t_diff_method}.  Therefore, we are motivated to investigate \textit{\textbf{how much training cost a tensor layer can reduce?}}

There are three main reasons for the high cost of pretraining LLMs: 1) a large number of parameters in LLMs; 2) the large memory footprint during the training; 3) the low GPU utilization during the training.

\textbf{Reduce the number of parameters in LLMs}

The linear layer accounts for more than $95\%$ of parameters in LLMs, which have a huge number of parameters. 
%We use the low-rank tensor layers to reduce the number of parameters by more than $10$ times.
%In LLMs, more than $95\%$ of the parameters are in the linear layer However, the size of linear layers grows with dimension squared, leading to a huge number of parameters in the LLM.
%As shown in Table \ref{table:s_t_diff_method}, a linear layer of size $n^4$ can be compressed by the CP layer to size $4nr$, that $n$ is the dimension of the LLM and $r$ is the rank of the CP layer. 
For example, Llama-70B \cite{llama2} has $70$B parameters, and there are $68$B parameters in linear layers, accounting for $98\%$ of the total parameters. In our method, we use the low-rank layers in Section \ref{sec:tensor_layer} to replace the linear layers in LLMs. For an LLM with dimension=$4,096$, each linear layer has $16.8$M parameters. With rank=$8$, each low-rank matrix layer has $65.5$ thousand parameters. The size of the linear layer can be reduced by more than $99\%$, and the entire model size can be reduced by about $95\%$.

%For an LLM with dimension=$4,096$, each linear layer has a weight matrix $\bm{W} \in \mathbb{R}^{4096 \times 4096}$, which has $16.8$M parameters. With rank=$8$, each low-rank matrix layer has two weight matrices $\bm{W_{rl1}} \in \mathbb{R}^{4096 \times 8}$ and $\bm{W_{rl2}} \in \mathbb{R}^{8 \times 4096}$, which has $65.5$ thousand parameters.

%In this method, we train an LLM from scratch by replacing the linear layer in (\ref{eq:linear_layer}) with different low-rank tensor layers in Section \ref{sec:tensor_layer}. For example, all linear layers (\ref{eq:linear_layer}) are replaced by a pair of two matrices in (\ref{eq:low_rank_layer}), whose size is $2n^2r$ and involves $2n^2r$ multiplications. The training cost of an LLM is expected to be significantly reduced.

%\textbf{bottleneck}: Training an LLM takes a lot of time.
%as given in Table \ref{table:s_t_diff_method}. In LLM, the computation cost of linear layers accounts for about $80\%$.

\textbf{Reduce GPU memory footprint during the training}

The GPU memory footprint of training LLMs typically exceeds hundreds of gigabytes. As shown in Fig. \ref{fig:GPUmemoryforllama}, the GPU memory footprint during the training consists of two main components, intermediate outputs and optimizer states. 1) The low-rank tensor layers have the same output size as linear layers, but fewer computations as shown in Table \ref{table:s_t_diff_method}. Using intermediate outputs recomputation as in Sec.\ref{sec:inter_out_rec}, the GPU memory footprint can be significantly reduced, at the cost of a few computations. For example, Llama2-70B \cite{llama2} has a model size of $140$ GB. Training this model has intermediate outputs size of $485$ GB for each batch of data. The memory footprint of intermediate outputs is reduced from $485$ GB to $5$ GB or $30$ GB, with $33\%$ or $5\%$ increase in computation as a trade-off. 2) The remaining GPU memory footprint consists mainly of parameters, gradients, and optimizer states, which have the size of $140$ GB, $140$ GB, and $840$ GB, respectively. Using optimizer state optimization as in section.\ref{sec:opt_sta}, there are $980$ GB of GPU memory footprint that be divided equally among multiple GPUs.
%\textcolor{red}{we can reduce the GPU memory footprint of these data from $1,120$ GB to $140+\frac{980}{n}$ GB in data parallelism training with $n$ GPUs.}

%As $n$ increases, the GPU memory footprint during the training will approach $140$ GB, still exceeding the memory capacity of a single GPU. During the training, the LLM is loaded on multiple GPUs. The training for model parallelism can be accelerated with the pipeline method as in Sec. \ref{sec:pipeline_model_parallel}.
\textbf{Improving GPU utilization during training}
GPU utilization is low in two ways, 1) GPUs have long idle times; 2) GPU throughput is much lower than peak performance.

During the training, the bandwidth of the disk is a bottleneck, and only one GPU is working at the same time in the model parallel as shown in \ref{fig:modelparallel}. Training datasets of LLMs have a large scale, as shown in Table \ref{table:llm_pandt}. During the training, datasets first load from disk to CPU memory, then transfer from CPU to GPU memory. However, the transfer bandwidth between CPU memory and GPU memory is $32.5$ GB/s, and the bandwidth of the disk ranges from $600$ MB/s to $4$ GB/s. In our method, we prefetch data batches by overlapping the data transfer and GPU computing during the training. When the LLM training on a batch of data, we load the data required for subsequent iterations from disk to CPU memory. For model parallel, we further split the training data in CPU memory into multiple sub-data as shown in Fig. \ref{fig:pipeline}.

In pre-training, the weights are initialized to full-precision floating point numbers. However, full-precision models are still large and can not fully utilize the GPU tensor cores for computation. Our method quantizes the full-precision(32-bit) parameters into half-precision(16-bit). As shown in Table \ref{table:mm_time}, the GPU performance when computing half-precision data is $16$ times better than computing full-precision data. {summaries: about model size and inference}).

%For example, Llama2-7B \cite{llama2} has a model size of $14$ GB. Training this model has intermediate outputs size of $96$ GB for each batch of data. The memory footprint of intermediate outputs is reduced from $96$ GB to $1$ GB, with a $33\%$ increase in computation as a trade-off.

%We use the virtual GPU memory to reduce the GPU memory requirements and use the pipeline method to improve the efficiency of model parallelism.

%The training starts with directly initializing. And the model keeps the low-rank structure during the training. We use the pipeline model parallel to train our model. 

%In this method, we represented the linear layer in the large language model as the low-rank matrix or tensor layer in Section \ref{sec:tensor_layer}. Then we get a model with fewer parameters, and we train this model from scratch.

%We initialize a large language model, which has the tensor layer in Section \ref{sec:tensor_layer} instead of the linear layer as (\ref{eq:linear_layer}). The model size is reduced more than 20 times compared to the original model. And the data type of parameters in this model is set to half-precision floating-point (FP16). 

%We train the model using the pipeline model parallelism. 

%For the low-rank matrix, we have two weight matrices $\bm{A} \in \mathbb{R}^{r \times n}$ and $\bm{B} \in \mathbb{R}^{m \times r}, r \ll min(n, m)$, and input matrix $\bm{X} \in \mathbb{R}^{n \times b}$ with batch-size = b.

% We split matrix $\bm{A}$ and $\bm{B}$ into some blocks with size of $8 \times 4$, and split matrix $\bm{X}$ into some blocks with size of $4 \times 8$. Then $\bm{A}$ be split into $\frac{r}{8} \times \frac{n}{4}$ blocks, $\bm{B}$ be split into $\frac{m}{8} \times \frac{r}{4}$ blocks, $\bm{C}$ be split into $\frac{n}{4} \times \frac{b}{8}$ blocks.

%We need a pretrained large language model in Section \ref{section:two_stage}, which means a high training cost.

%Reducing training costs because the model size is much smaller.

\begin{figure}[t]
\centering
\includegraphics[width=8cm]{figs/fd_learning.png}
\caption{Federated Learning.}
\label{fig:fd_learning}
\end{figure}

\subsection{Method 4: Federated Learning}

%In the era of LLM, data privacy is a very important issue.
Training an LLM takes a large amount of real corpus data, which has raised concerns about data privacy. For example, OpenAI is getting sued for illegally using content from the internet to train their LLM (chatGPT) \cite{chatGPTintrouble}. Some industries or companies stored their own data at local nodes. They need to protect the privacy of their data when training an LLM collaboratively.
% \begin{itemize}
%     \item highly data collection cost,
%     \item competitive reasons,
%     \item confidentiality or privacy concerns.
% \end{itemize}
%Industries, such as healthcare and legal, cannot share users' data, due to confidentiality or privacy concerns. 

Federated learning \cite{fdlearning} provides a practical solution for collaboratively training LLMs. It protects training data from leakage by distinguishing between global training and local training \cite{yang2021recommendations}. In federated learning, the raw data is distributed stored, and trained at multiple local nodes, the gradients with the same size as the model are exchanged among computing nodes at each Iteration, resulting in huge communication overhead. Therefore, we are motivated to investigate \textit{\textbf{how much communication overhead a tensor layer can reduce?}}

As shown in Fig. \ref{fig:fd_learning}, using federated learning to train an LLM, each iteration consists of three steps as follows:
\begin{enumerate}
    \item  A center node (like a parameter server\cite{li2014communication}) broadcasts the latest LLM to other computing nodes. 
    \item  Each computing node trains it on its local data to obtain the gradients, which are sent back to the center node. 
    \item The center node gathers these gradients to update the global LLM using some average schemes. 
\end{enumerate}
For example, training the Llama2-7B model \cite{llama2}, which has a model size of $14$ GB, takes $296$K iterations. Using $4$ nodes to train the model by federated learning, center node-0 communicates with each node twice in step-1 and step-3 per iteration. And in an iteration, the communication overhead of the central node and each computing node is $84$ GB and $28$ GB respectively. For the entire training, the communication overhead is $24$ PB and $8$ PB. Federated learning transfer data on the web, which normally achieves $10 \sim 100$ MB/s bandwidth. These communications have a significant time cost.

The considerable communication overhead in federated learning is due to the large parameter size of the LLMs. Note that training from the LoRA method has much fewer trainable parameters than the original LLM.

In this method, we use low-rank adaption training as in Section \ref{sec:lora} for federated learning, and each iteration consists of four steps as follows:
\begin{enumerate}
    \item Each node has the same pretrained weights and freezes them.
    \item The center node broadcasts the trainable low-rank factors $\mathbf{A} \in \mathbb{R}^{n^2 \times r}$ and $\mathbf{B} \in \mathbb{R}^{r \times n^2}$ as in (\ref{eq:low_rank_layer}) to other nodes.
    \item Each node train the low-rank weights $\mathbf{A}$ and $\mathbf{B}$ on their local data. They obtain the gradients of these trainable parameters, which have the same size as low-rank factors.
    \item Each node sends gradients back to the center node, which gathers these gradients to update the global low-rank factors.
\end{enumerate}
After the training, the center node broadcasts the global trainable low-rank factors to other nodes. These nodes merge the low-rank factors with pretrained weights as (\ref{eq:new_linear_layer}).

In step-2 and step-4, our federated learning transfers the low-rank layers. For training the LLaMA-7B model with $4$ nodes, LR layers, CP layers, and TT layers reduce the communication overhead of the center node from $84$ GB to $50.4$ MB, $1.56$ MB, and $7.08$ MB, respectively in each iteration. The time cost of data communication is about one second. For the entire training, the communication overhead of the center node is reduced from $24$ PB to $15$ TB, $0.46$ TB, and $2$ TB respectively. 

%The communication overhead would be $102$PB between the center node with each computing node. Low-rank tensors can reduce the communication overhead from 102PB to less than 5PB.

%For example, training the LLaMA-65B model \cite{touvron2023llama}, which has a model size of $130$ GB, takes $414$K iterations. 

%In the method, we train a LLM by replacing the linear layer in (\ref{eq:linear_layer}) with different low-rank tensor layers in Section \ref{sec:tensor_layer} using federated learning. The tensor layer-based LLM has a much smaller size, as given in Table \ref{table:s_t_diff_method}. In the training stage, the gradient has the same size as tensor layer-based LLM. The communication overhead is expected to be significantly reduced.
%LLama 0.41375 million batch%
